MultiRef: Controllable Image Generation with Multiple Visual References

Visual designers naturally draw inspiration from multiple visual references, combining diverse elements and aesthetic principles to create artwork. However, current image generative frameworks predominantly rely on single-source inputs -- either text prompts or individual reference images. In this paper, we focus on the task of controllable image generation using multiple visual references. We introduce MultiRef-bench, a rigorous evaluation framework comprising 990 synthetic and 1,000 real-world samples that require incorporating visual content from multiple reference images. The synthetic samples are synthetically generated through our data engine RefBlend, with 10 reference types and 33 reference combinations. Based on RefBlend, we further construct a dataset MultiRef containing 38k high-quality images to facilitate further research. Our experiments across three interleaved image-text models (i.e., OmniGen, ACE, and Show-o) and six agentic frameworks (e.g., ChatDiT and LLM + SD) reveal that even state-of-the-art systems struggle with multi-reference conditioning, with the best model OmniGen achieving only 66.6% in synthetic samples and 79.0% in real-world cases on average compared to the golden answer. These findings provide valuable directions for developing more flexible and human-like creative tools that can effectively integrate multiple sources of visual inspiration. The dataset is publicly available at: https://multiref.github.io/.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\ranjay}[1]{{\color{orange}#1}}
\newcommand{\peter}[1]{{\color{olive}#1}}

\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
\PassOptionsToPackage{table,dvipsnames}{xcolor}  % 先把选项“下发”给 xcolor
\RequirePackage{xcolor}  
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}
\usepackage{xspace}
\usepackage{colortbl}

\newcommand{\dataset}{\textsc{MultiRef}\xspace}
\newcommand{\benchmark}{\textsc{MultiRef-bench}\xspace}
\newcommand{\engine}{\textsc{RefBlend}\xspace}
\newcommand{\header}[1]{\smallskip \noindent\textbf{{#1}}\xspace}

\usepackage{bbding}
\usepackage{pifont}
 \usepackage{multirow} 
 \usepackage{threeparttable}
 \usepackage{subcaption}
 % 在导言区只保留这一处

\usepackage[most]{tcolorbox}

%  \usepackage[table]{xcolor}
% \usepackage[most]{tcolorbox}
% \usepackage{xcolor}
 \usepackage{tikz}
 \usepackage{enumitem}
 \usepackage{array}
 % \usepackage{titlesec}
 \usepackage{booktabs}
% \definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
% \usepackage[pagebackref,breaklinks,colorlinks,allcolors=cvprblue]{hyperref}
\newcommand{\xmarkcolor}{%
  \textcolor{red}{%
    \begin{tikzpicture}[scale=0.2]
      \draw [line width=1.5] (0,0) -- (1,1);
      \draw [line width=1.5] (1,0) -- (0,1);
    \end{tikzpicture}%
  }%
}

\newcommand{\checkmarkcolor}{
    \tikz[baseline=(checkIcon.base)]{
        \node[draw=gray!30,line width=0.5pt, fill=green!70!black,rounded corners,inner sep=1.5pt] (checkIcon) {\textcolor{white}{$\checkmark$}};
    }
}
\usepackage[most]{tcolorbox}
\definecolor{modelcolor1}{HTML}{d0e0e3}
\definecolor{modelcolor2}{HTML}{dad2e9}
\definecolor{modelcolor3}{HTML}{fce5cd}
\definecolor{opensourcecolor}{HTML}{b4c8b6}
\definecolor{commercialcolor}{HTML}{fadadd}
\tcbset{
    prompt/.style={
        colback=gray!10!white,
        colbacklower=gray!20!white,
        colframe=white,
        boxrule=0.5mm,
        left=1mm,
        right=1mm,
        top=1mm,
        bottom=1mm,
        arc=1mm,
        boxsep=3mm,
        drop shadow={black!50!white}, 
        enhanced,
        boxed title style={
            colback=cyan!50!black,
            colframe=cyan!50!black,
            fontupper=\bfseries, 
            size=small,
            boxsep=3pt
        },
        coltitle=white, % 使用标题颜色设置
        attach boxed title to top left={yshift=-\tcboxedtitleheight/2, xshift=5mm},
    }
}
\definecolor{TealBlue}{RGB}{54,117,136}      % matplotlib "teal"
\definecolor{OliveGreen}{RGB}{107,142,35}    % matplotlib "olive"
\definecolor{SeaGreen}{RGB}{46,139,87}       % matplotlib "seagreen"
\definecolor{Cerulean}{RGB}{42,82,190}       % matplotlib 接近 "cerulean"
\definecolor{MidnightBlue}{RGB}{25,25,112}   % matplotlib "midnightblue"
\definecolor{Periwinkle}{RGB}{197,203,255}   % matplotlib 接近 "periwinkle"
\definecolor{RoyalPurple}{RGB}{120,81,169}   % matplotlib "mediumpurple"/royal purple
\definecolor{Fuchsia}{RGB}{255,0,255}        % matplotlib "fuchsia"/magenta

==> sec/5_discussion.tex <==
\section{Discussion}

==> table/small-real-results.tex <==
\begin{table}[!ht]
  \centering
  \setlength{\tabcolsep}{6pt}
  \caption{Real-world image generation conditioned on multiple image references (Overall performance). Although today's image generative models produce high-quality outputs, most struggle with accurately following instructions and maintaining fidelity to source images. \textbf{IQ} - Image Quality, \textbf{IF} - Instruction Following, \textbf{SF} - Source Fidelity.}
  \label{tab:small-real+mllm-judge-overall}
  \vspace{-1em}
  \begin{tabular}{l|ccc}
    \toprule[1.5pt]
    \textbf{Model} & \textbf{IQ} & \textbf{IF} & \textbf{SF} \\
    \midrule
    \multicolumn{4}{c}{\textcolor{violet!80!white}{\cellcolor{gray!10!white} \textbf{\textit{Unified Model}}}} \\ \midrule 
    Show-o & 0.513 & 0.293 & 0.254 \\
    OmniGen & \underline{0.555} & \underline{0.496} & \underline{0.421} \\
    ACE & 0.254 & 0.205 & 0.203 \\
    \midrule
    \multicolumn{4}{c}{\textcolor{violet!80!white}{\cellcolor{gray!10!white} \textbf{\textit{Compositional Framework}}}} \\ \midrule 
    ChatDiT & 0.657 & 0.445 & 0.375 \\
    Gemini+SD2.1 & 0.614 & 0.412 & 0.342 \\
    Claude+SD2.1 & 0.638 & 0.423 & 0.345 \\
    Gemini+SD3 & 0.744 & 0.583 & 0.464 \\
    Claude+SD3 & 0.742 & 0.569 & 0.447 \\
    Gemini+SD3.5 & \textbf{0.774} & 0.588 & \textbf{0.467} \\
    Claude+SD3.5 & 0.765 & \textbf{0.589} & 0.462 \\ \midrule
    \rowcolor{gray!10!white} Ground Truth & 0.733 & 0.767 & 0.706 \\
    \bottomrule[1.5pt]
  \end{tabular}
  \vspace{-1em}
\end{table}

==> table/synthetic-judge-eval.tex <==
\begin{table*}[!ht]
\centering
\caption{Our fine-tuned MLLM-as-a-Judge scoring align closely with human preferences in assessing semantic-level visual reference.}
\label{tab:eval judges in synthetic data}
\vspace{-1em}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc}
\toprule[1.5pt]
\multirow{2}{*}{\textbf{Condition Type}} & \multicolumn{2}{c|}{\textbf{Subject}} & \multicolumn{2}{c|}{\textbf{Depth}} & \multicolumn{2}{c|}{\textbf{Caption}} & \multicolumn{2}{c|}{\textbf{Mask}} & \multicolumn{2}{c|}{\textbf{Style}} & \multicolumn{2}{c|}{\textbf{Sketch}} & \multicolumn{2}{c}{\textbf{Semantic Map}} \\
 & Pearson & MAE & Pearson & MAE & Pearson & MAE & Pearson & MAE & Pearson & MAE & Pearson & MAE & Pearson & MAE \\
\midrule
Sample Size & \multicolumn{2}{c|}{158} & \multicolumn{2}{c|}{358} & \multicolumn{2}{c|}{169} & \multicolumn{2}{c|}{74} & \multicolumn{2}{c|}{158} & \multicolumn{2}{c|}{276} & \multicolumn{2}{c}{154} \\
\midrule
\rowcolor{gray!10!white} GPT-4o-mini & 0.759 & 0.779 & 0.367 & 1.592 & 0.782 & 0.580 & 0.390 & 1.662 & 0.457 & 0.949 & 0.490 & 1.290 & 0.404 & 1.188 \\
Qwen-2.5-2b-vl-zs & 0.231 & 1.475 & 0.044 & 1.631 & 0.864 & 0.491 & 0.051 & 1.987 & 0.173 & 2.671 & 0.239 & 1.446 & 0.209 & 1.338 \\
Qwen-2.5-7b-vl-zs & 0.694 & 0.892 & 0.148 & 1.757 & 0.869 & 0.515 & 0.495 & 1.757 & 0.293 & 1.171 & 0.270 & 1.515 & 0.618 & 1.117 \\
\textbf{Qwen-2.5-2b-vl-ft (ours)} & \textbf{0.726} & \textbf{0.722} & \textbf{0.581} & 0.944 & 0.853 & 0.509 & 0.386 & 1.216 & 0.402 & 0.949 & 0.567 & 1.007 & 0.622 & 1.124 \\
\bottomrule[1.5pt]
\end{tabular}}
\vspace{-1em}
\end{table*}
